Improved Inference of Human Intent by Combining Plan Recognition and Language Feedback

Conversational assistive robots can aid people, especially those with cognitive impairments, to accomplish various tasks such as cooking meals, performing exercises, or operating machines. However, to interact with people effectively, robots must recognize human plans and goals from noisy observations of human actions, even when the user acts sub-optimally. Previous works on Plan and Goal Recognition (PGR) as planning have used hierarchical task networks (HTN) to model the actor/human. However, these techniques are insufficient as they do not have user engagement via natural modes of interaction such as language. Moreover, they have no mechanisms to let users, especially those with cognitive impairments, know of a deviation from their original plan or about any sub-optimal actions taken towards their goal. We propose a novel framework for plan and goal recognition in partially observable domains -- Dialogue for Goal Recognition (D4GR) enabling a robot to rectify its belief in human progress by asking clarification questions about noisy sensor data and sub-optimal human actions. We evaluate the performance of D4GR over two simulated domains -- kitchen and blocks domain. With language feedback and the world state information in a hierarchical task model, we show that D4GR framework for the highest sensor noise performs 1% better than HTN in goal accuracy in both domains. For plan accuracy, D4GR outperforms by 4% in the kitchen domain and 2% in the blocks domain in comparison to HTN. The ALWAYS-ASK oracle outperforms our policy by 3% in goal recognition and 7%in plan recognition. D4GR does so by asking 68% fewer questions than an oracle baseline. We also demonstrate a real-world robot scenario in the kitchen domain, validating the improved plan and goal recognition of D4GR in a realistic setting.

==> evaluation_two_domain.tex <==
\section{Evaluation}

Our evaluation aims to test the hypothesis that our multi-modal decision-theoretic framework DGR-POMDP improves 1) the accuracy of goal recognition and plan recognition  of human activity and 2) the robot's ability to guide the person towards task success
\nnote{the expected return in guiding the user in completing the tasks successfully by observing the human actions and strategically asking clarification questions and instructing the human when the feedback is opposite to robot's own belief. }
% \stnote{2 is very wordy.  can you condense or simplify?  Here is an attempt:  the robot's ability to guide the person towards task success} 
We measure the enhanced performance of our algorithm by measuring the accuracy of goal recognition and plan recognition at every time step. We also measure the planning time, the cumulative expected return and the number of clarification questions asked for completing the task.
% , and \iinote{??}

% goal recognition (Human Intent Recognition) by observing the human actions and strategically asking clarification questions is better than 1) asking random questions and 2) just passively observing the human actions.

\subsection{Virtual Home  Simulation}
We use the simulation environment introduced by 
% \stnote{Does it have an official name? a little weird tor efer to it only by citation number}\iinote{?ask} 
\citep{wang2017hierarchical} as a testbed for simulation experiments of D4GR. 
The simulator models real environment state changes that result from  executed steps from a virtual human. There are 18 binary virtual sensors corresponding to the object's attributes and state of smart home sensors some of the examples inclue \iinote{add this. \iinote{The list of all the sensors is added in the supplementary section}. The simulator controls the occurrence of predefined human actions. The reliability of the sensors varies from 99\% to 80\%, and the difficulty of the environment changes as a human tries to move from doing a single task with correct steps to doing multiple tasks with wrong actions.

\subsection{Domains and Experiment Test Cases}
We test our algorithm in two domains - Kitchen and block. - The Knowledge Base, $TaskNet$ of the HTN for kitchen has three goals: wash hands, make tea, and make coffee. While the block domain h The knowledge graph used for our experiments is shown in Fig-\ref{Fig-htn}. These are three tasks that humans can do in our simulated environment. We experiment over four categories of test case scenarios:
\begin{itemize}
    \item the easiest problem category \textbf{p1 - Single Goal and Correct Steps}, captures scenarios where the human takes correct step sequences for achieving a single goal. 
    \item \textbf{p2 - Multiple Goals Correct Step}. The human actions in these cases indicate that a person works on many goals simultaneously by switching back and forth,
    \item \textbf{p3 - Single Goal with Wrong Step} where a human does single goal but with probability C in Eq-\ref{eq:currstep-transition} as introduced in  executes a wrong steps 
    \item The hardest problem category \textbf{p4 - multiple goals and wrong steps} where human moves back and forth between goals and also executes wrong actions. 
\end{itemize}

%% Examples of the test cases for each category are shown in  Fig-\ref{Fig-testcase}. For this paper, wrong human steps are divided into non-related wrong steps and related wrong actions, depending on whether a wrong step changes the carry-on effects of its previous actions hence affecting the current goal status. In p3 of Fig-\ref{Fig-testcase}, underlined "use-soap" is a non-related step as it causes a sub-optimal trajectory as it takes longer the human to complete the task. Still, this human action itself does not have any impact on
%% the carry-on effects of the previous steps. \nsnote{This previous sentence could be broken up into two sentences} On the other hand, the underlined "turn\_off\_faucet" is a related wrong step because it changes the faucet state from on to off, which is a carry on effect of the previous actions. We set C = 0.837 same as the authors in \citep{wang2017hierarchical}.  The simulator, given a test case, simulates step by step changes of objects' states and sensor measurements, with consideration
%% of sensor reliability.

%% \begin{figure}[t]
%%     \centering
%%     \includegraphics[width=0.8\linewidth]{images/test_casse.png} 
%%     \caption{Example Test Case for Each Category -  washing hands, making tea, and making coffees\cite{wang2017hierarchical}}
%%     \label{Fig-testcase}
%%     \end{figure}

% \subsection{Case Study Data Collection}
% \iinote{Tian Add}


